Neural Compression of Atmospheric States

Atmospheric states derived from reanalysis comprise a substantial portion of weather and climate simulation outputs. Many stakeholders -- such as researchers, policy makers, and insurers -- use this data to better understand the earth system and guide policy decisions. Atmospheric states have also received increased interest as machine learning approaches to weather prediction have shown promising results. A key issue for all audiences is that dense time series of these high-dimensional states comprise an enormous amount of data, precluding all but the most well resourced groups from accessing and using historical data and future projections. To address this problem, we propose a method for compressing atmospheric states using methods from the neural network literature, adapting spherical data to processing by conventional neural architectures through the use of the area-preserving HEALPix projection. We investigate two model classes for building neural compressors: the hyperprior model from the neural image compression literature and recent vector-quantised models. We show that both families of models satisfy the desiderata of small average error, a small number of high-error reconstructed pixels, faithful reproduction of extreme events such as hurricanes and heatwaves, preservation of the spectral power distribution across spatial scales. We demonstrate compression ratios in excess of 1000x, with compression and decompression at a rate of approximately one second per global atmospheric state.

==> 00_abstract.tex <==
Atmospheric states derived from reanalysis comprise a substantial portion of weather and climate simulation outputs. Many stakeholders --- such as researchers, policy makers, and insurers --- use this data to better understand the earth system and guide policy decisions. Atmospheric states have also received increased interest as machine learning approaches to weather prediction have shown promising results. A key issue for all audiences is that dense time series of these high-dimensional states comprise an enormous amount of data, precluding all but the most well resourced groups from accessing and using historical data and future projections. To address this problem, we propose a method for compressing atmospheric states using methods from the neural network literature, adapting spherical data to processing by conventional neural architectures through the use of the area-preserving HEALPix projection.
We investigate two model classes for building neural compressors: the hyperprior model from the neural image compression literature and recent vector-quantised models.
We show that both families of models satisfy the desiderata of small average error, a small number of high-error reconstructed pixels, faithful reproduction of extreme events such as hurricanes and heatwaves, preservation of the spectral power distribution across spatial scales.
%High-performance multi-decadal atmospheric compression methods have up to this point been missing in the field.
We demonstrate compression ratios in excess of $1000\times$, with compression and decompression at a rate of approximately one second per global atmospheric state.


%%%% RECENT COMMENTS

% These problems will be exacerbated by increasing the resolution, the number of years, and the number of scenarios of Earth System Models. %higher-resolution climate projections, where 100-year data of different scenarios and models increase the amount to data. 

%such that a larger audience can access and process such data efficiently.

%(MAE around 0.4$^\circ$~K for temperature, around $0.5~\text{m}/\text{s}$ for zonal and meridional wind, below 100 Pa for surface pressure and around $40~\text{m}^2/\text{s}^2$ for geopotential), 

%To our knowledge, this is the first work that studies neural compression at a multi-decadal scale with a high compression rate of $1000\times$ and above, and that aims at releasing the compressed outputs for use by the community.\todo{CRA5? Also, under-promise and over-deliver?}
%We provide our open source code and compressed outputs for use by the community.\dwf{Should this line be in the initial arXiv version if the release is not simultaneous?}


%%%%% THIS IS OLD

%Atmospheric data comprise a large percentage of the output generated by both weather and earth system (climate) models. Such data have been important historically to researchers study of effects of dynamics , but has also received increased researcher attention %have now also viewed this data with an increasing level of interest as 
%for training machine-learning surrogates of atmospheric dynamical models. % A key component of these surrogate models
% are approaching the quality of traditional simulation systems
% are the large corpora on which they are trained. 
%Such corpora, however, pose significant engineering challenges as the data are extremely large
%One challenge for using these datasets are simply its size: for instance, 40 years of 0.25 degree data at 1 hour timesteps requires 250TB of storage. Such requirements preclude all but the most well resourced groups to tackle such problems. In fact, even transferring such data incurs a significant cost.

%We aim to lower the barrier to entry by learning compressed representations of atmospheric states, with the goal of lowering storage needs, more quickly transferring data, and perhaps reducing the accelerator requirements for learning ML surrogates. We investigate two classes of models -- the hyperprior and VQ-VAE/GAN -- for neural compression, with the desiderata that: 1) the average error is small, 2) the maximum error is bounded, 3) error on extreme values is limited, and 4) spectral properties are preserved. We find that, with the appropriate choice of grids and models, that we are able to compress atmospheric data that satisfy these desiderata by a factor of 1000X \emph{obv, this number should change, and the writing is weird}. Further, we open-source the code for use by the community, and store compressed representations of ERA5 data to enable fast transfer. Moreover, to the best of our knowledge, this is the first large-scale study on neural compression on a large corpus of high-resolution data.

==> 01_introduction.tex <==
\section{Introduction}
\label{sx:introduction}

This paper presents a family of neural network compression methods of simulated atmospheric states, with the aim of reducing the currently immense storage requirements of such data from cloud scale (petabytes) to desktop scale (terabytes). 
%This need for new types of compression methods is motivated by the ubiquitous role that environmental data plays in scientific, industrial, and policy-level disciplines. As datasets increase in size and complexity to meet the demands of these diverse areas, the need for more effective storage and use, and consequently the need for more efficient and bespoke compression solutions, has become more urgent and necessary.
%
%Among the use cases for the data is improving our understanding of our planet at climate multi-decadal temporal scale, understanding the history of the planet's climate, weather forecasting, modeling environmental disasters, and reaching agreements over CO$_2$ reduction. 
This need for compression has come about over past 50~years, characterized by a steady push to increase the resolution of atmospheric simulations, increasing the size and storage demands of the resulting datasets (e.g., \citet{neumann2019assessing}, \citet{schneider2023harnessing}, \citet{essd-16-2113-2024}), while atmospheric simulation has come to play an increasingly critical role in scientific, industrial and policy-level pursuits.
Higher spatial resolutions unlock the ability of simulators to deliver more accurate predictions and resolve ever more atmospheric phenomena.
%, and such simulators have come to play a critical role in scientific, industrial, and policy-level disciplines.
For example, while current models often operate at 25 - 50~km resolution, resolving storms requires 1~km resolution~\citep{stevens2020added}, while resolving the motion of (and radiative effects due to) low clouds require 100~m resolution~\citep{schneider2017earth,satoh2019global}.
%Increasing spatial resolution is also key to improving the temporal prediction quality of physics-based models.
Machine learning models for weather prediction also face opportunities and challenges with higher resolution: while additional granularity may afford better modeling opportunities, even the present size of atmospheric states poses a significant bottleneck for loading training data and serving model outputs~\citep{chantry2021opportunities}.
%Across weather and climate fields, as data sizes have increased, the need for more effective storage and use, and consequently, the need for more efficient and bespoke compression solutions, has become more urgent and necessary.

%This current size of atmospheric states motivates the need for compression. 
To put the data storage problem in perspective, storing 40 years of reanalysis data from the ECMWF Reanalysis v5 dataset (ERA5, \citet{hersbach2020era5}) at full spatial and temporal resolution (i.e.\ without subsampling)
%complement of 137 elevation levels, at 0.25$^\circ$ (28~km at equator) spatial resolution and 1~hour temporal resolution~
requires 181~TB of storage per atmospheric variable.
For 6 such variables, a single trajectory exceeds 1~PB, to say nothing of an ensemble of tens or hundreds of trajectories as required for model intercomparison or for predicting distributions of outcomes~\citep{eyring2016overview}. %, as with climate models.
As \citet{sz3_framework} write, ``recent climate research generates 260 TB of data every 16s''. %\citep{foster2017computing}.
%
Such conditions create considerable difficulties, prompting researchers to discard data or decrease temporal and/or spatial resolution. 
%has prompted those developing weather models to discard data, either by decreasing the temporal resolution (as done with the GraphCast \citep{lam2023graphcast} and GenCast \citep{price2023gencast} models) or decreasing the spatial resolution, as in earlier weather forecasting work by \citet{keisler2022forecasting} or \citet{weyn2020improving}.
%, or limiting the number of steps in multi-step loss (GC, everything else). % Commenting this out, since unlike the previous two examples, this doesn't seem like an example of sidestepping data size problems.
%
% Resorting to these methods led to decreased specificity of model predictions and performance of models.
Having to decimate the dataset to satisfy financial and engineering constraints is especially unfortunate for machine learning models, whose performance is often bounded by the size of the training dataset,
while also making fair and systematic comparisons to results from traditional numerical weather prediction (NWP) more challenging.
%
%Modifying the dataset resolution 
%
% These problems of data size become only more acute for climate projection, which can generate multiple sequences of atmospheric states, one for each model or scenario, with each sequence spanning 100 years. 
Perhaps most importantly, the size of the data precludes access to the full dataset for all but the most well-resourced groups. % to create state-of-the-art models.
Priced at the time of writing, cloud storage for 100 PB costs on the order of \$1M per month\footnote{This value was obtained by looking up the publicly available rate for cloud storage fees on 28 June 2024 from two of the large cloud storage providers. Costs depend on data replication and access requirements.}.

Data compression is a well-studied problem with many off-the-shelf algorithms available. Unfortunately, for continuous-valued data such as atmospheric states, modern lossless compression methods tailored to such data offer only modest savings, reducing the size by only a factor of 2  (c.f. Figure \ref{fig:reprojection_error_vs_cr_bounded_compression}). Existing lossy compression algorithms pose their own problems, as they are usually designed to compress while optimizing mean squared error~(MSE)~\citep{sz3_algo}.
In the weather and climate domain, the MSE loss in particular can attenuate high spatial frequencies and thereby remove physically important spatial discontinuities~\citep{ravuri2021nowcasting}. % vs "sharp features"
%
%In psychophysical domains such as images, sound and video, specialized algorithms ensure that distortions manifest only in forms that are minimally perceptible to human senses~\citep{wallace1992jpeg}.
Na\"ive pursuit of reduced MSE can result in significant, scientifically problematic distortions, including outright erasure of entire hurricanes as noted in \cite{huang2022compressing}. This motivates the development of bespoke compression methods evaluated with an eye towards not just MSE but also other physical metrics of scientific interest, such as power spectrum distortion and the preservation of extrema.

%Atmospheric data has received an increasing level of interest for both weather- and climate-related problems. Much of this increased interest is driven by machine-learning approaches to weather prediction. The rapid improvement of these models have led researchers to speculate if one can apply such approaches to climate projection. A key component of ML models are large corpora of data that are used to train models. Unfortunately, the size of these datasets are extremely large; for instance, storing 40-years of 0.25-deg data at 1-hour temporal resolution requires 250TB of storage. The size of such datasets preclude all but the most well-resourced groups from operating as such a resolution, with less well-resourced researchers relegated to operating at vastly reduced spatial and temporal resolutions. Such hindrances slow down the progress of research by limiting the number of researchers on the problem. Moreover, these problems will become only more acute when we look to climate projections, where 100-year data of different scenarios and models increase the amount to data.

% vs "neural compressor" - we say nothing about neural anything to this point
%At a practical level, we aspire to
%We aim to bridge this gap by learning compressed representations of the atmosphere to 
%reduce storage requirements from cloud scale (PB) to desktop scale (TB), enabling researchers to use atmospheric datasets in full without need of discarding data. Such compression also speeds up data transfer at all levels, from sharing results between researchers to increasing data throughput when training a model.
%At a scientific level, our results illustrate the degree of informational redundancy in atmospheric states. 

% This whole paragraph seems like a bit of a strawman. Cut?
% At first glance, learning compression of atmospheric states seems infeasible as we aim to learn a low-dimensional representation of 67$M$-dimensional atmospheric states from fewer than 100$K$ examples \footnote{Each atmospheric state is $720 \times 1440 \times 13 \times 5$ at 1 hour temporal resolution for 40 years}. To compare this data to a standard image corpus, the dimensionality of each atmospheric state is greater than 900$\times$ larger than 256$\times$256 ImageNet and LAION-400M data, while containing 10$\times$ (ImageNet) and 10K$\times$ fewer examples. Recent work on AI weather prediction, however, suggests that compression is possible: well-performing models are trained on fewer than 40K examples and have, by modern standards, relatively few parameters (typically fewer than 500M parameters). Such a result suggests that the data is quite regularly structured and easily compressible. Further, preliminary results on unlearned compression on one atmospheric state\citep{klower2021compressing} and implicit neural representations for smooth fields such as geopotential \citep{huang2022compressing} provide further evidence.

% TODO[mkg]: move above data size comparison to Method:data section below. Replace it with an expansion of the "claims" section from the outline.
Based on the scientific, financial and social needs described above, suitable candidate compressors will be those capable of high compression rates, low error (both on average and for extreme values) and fast execution; %, which preserve physical and spatial consistency.
adequately meeting these needs will enable researchers to use atmospheric datasets in full without need of subsampling, increase the speed of data dissemination at all levels, and reduce storage costs.
In pursuit of this goal, we present a family of compression methods based on autoencoder neural networks that are adapted and trained for atmospheric data, and examine the inherent tradeoffs within this design space.
These compression methods illustrate and exploit the informational redundancy of atmospheric states.
In Section \ref{sx:learning2compress} we discuss existing compression methods and insight available in this area, and describe our own technical groundwork.
Within the family of methods we will describe, we will put forward a system based on the hyperprior model~\citep{balle2018hp} as the candidate neural compressor which most fully satisfies the requirements of atmospheric state compression.
As a case study, we showcase in Figure \ref{fig:hurricane_matthew_hyperprior} the compression results for hurricane Matthew, which shows low errors across physical variables of interest, as well as the ability to preserve extreme values and events.  

\input{figure_hyper_prior_hurricane_matthew}

Our overall approach comprises four stages, depicted in Figure \ref{fig:system}: reprojecting the atmospheric state to a square format better suited to ML accelerators using the HEALPix projection~\citep{gorski1999healpix}, employing a neural encoder to map these projections into a discrete representation (which can be losslessly compressed with standard techniques), reconstructing HEALPix projections using a neural decoder, and finally reprojecting back onto the equirectangular latitude/longitude grid using the spherical harmonics transform.

%We investigate two classes of models-—--hyperprior-based models and vector-quantized autoencoder models—--for neural compression, with the following desiderata:
%\begin{enumerate}
%    \item Small average errors (RMSE and MAE) \label{desiderata:mse}
%    \item Small number of high-error HEALPix pixels \label{desiderata:few_bad_cells}
%    \item Small error around extreme events \label{desiderata:extreme_events}
%    \item Preserves the spectral power distribution across spatial scales %\label{desiderata:spectral_error}
%    \item Fast encoding and decoding \label{desiderata:speed}
%\end{enumerate}


We will show in Section~\ref{sx:experiments} that our approach is able to compress these data at low error by approximately three orders of magnitude, and thus demonstrate bespoke high-compression methods applicable to multi-decadal data.
We obtain a mean absolute error (MAE) of approximately $0.4^\circ$~K for temperature, approximately $0.5~\text{m}/\text{s}$ for zonal and meridional wind, below 1 hPa for surface pressure and approximately $40~\text{m}^2/\text{s}^2$ for geopotential, with less than 0.5\% of HEALPix pixels beyond an error of $1^\circ$~K (temperature), $1~\text{m}/\text{s}$ (zonal and meridional wind) or less than 0.05\% of pixels beyond an error of $100~\text{m}^2/\text{s}^2$ (geopotential) while preserving spectral shape, and approximately one second encoding/decoding time per global state. 
We show that high-error pixels are rare enough that their values can be stored in a lookup table while keeping the overall compression ratio above 1000.
Because sharp features and rare events can be the first victim of aggressive compression, we conduct an analysis of weather events of interest such as hurricanes and heat waves to demonstrate that these are not distorted.
We provide a discussion of the different variations in use and further contextualisation of the results in Section \ref{sx:discussion}, and discuss limitations and conclude in Section \ref{sx:conclusion}.
%To our knowledge, this is the first work\footnote{Concurrent work on the compression of ERA5 data with similar errors and compression ratio of $230\times$ to $330\times$ has been published by \citep{han2024cra5}.} that studies neural compression of atmospheric states at a multi-decadal scale with high compression rate of $1000\times$.

%\footnote{We will soon release open-sourcing code and releasing compressed representations for use by the community.}

%

%Interest in weather prediction and climate projection has increased over the past few years, with promising results from machine learning models that are beginning to rival 
%
%One peculiarity of atmospheric data compared to image data is that the models that perform well on weather prediction are extremely small compared to the size of the dataset: a well-performing model such as GraphCast is less than 160MB for 6-hourly prediction (compared to 40TB of data). The dimensionality of each atmospheric state is 943x than 256x256 ImageNet and LAION-400M data
%
%\emph{these are only rough notes}
%Weather predictions and climate projections generate a tremendous amount of data. For instance, ECMWF generates XXXXTB of data per year. The atmospheric data generated as part of Earth System Models as part of CMIP6 is XXXX. Of course, this is daily subsampled data. (Say something about data being stored on tape). Design decisions led to these engineering challenges. Very high latency. ML has very different requirements. Need low latency, but not double precision. Cost on GCP.
%

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/overview_figure.pdf}
    \hfill
    \caption{Overview of our neural data compression system. Global surface and atmospheric data are projected onto the 12 HEALPix square base pixels. On the left, the figure illustrates 3 such squares, numbered 7 (in red, over the Indian Ocean), 10 (in green, over continental Europe and Arabic peninsula) and 11 (in blue, over East Asia), for $C$ variables (which may include different physical variables at one or multiple pressure levels), collected from a single atmospheric state at a given timestamp. We jointly compress $C$ separate channels for every $256 \times 256$ square into a quantized representation (here, we illustrate a $32 \times 32$ map of discrete VQ indices corresponding to a 4-downsampling-block VQ-VAE or VQ-GAN). During training and evaluation, we reconstruct the HEALPix squares back from compressed, quantized representations. After reconstruction, spherical harmonics coefficients are calculated via forward transform of the HEALPix reconstructions. These coefficients are used to synthesize re-projected images via inverse transform in latitude/longitude coordinates. On the right, the figure illustrates two re-projected reconstructions for variables 1 and $C$, with areas corresponding to different HEALPix squares coded in different colours. Metrics are computed during reconstruction (comparison of reconstruction vs. ground truth in HEALPix projection), after spherical harmonics forward transform (power spectrum) and after re-projection back onto latitude/longitude representations (comparison of re-projected reconstruction vs. ground truth in latitude/longitude coordinates).}
    \label{fig:system}
\end{figure}




==> 02_related.tex <==
\section{Learning to Compress}
\label{sx:learning2compress}

\subsection{Lossless and Lossy Compression}
\label{sx:methods:lossless-lossy}
Compression methods can be divided into \emph{lossless} and \emph{lossy} categories.
Lossless compression aims to transform data in such a way that the original can be reinstantiated exactly.
As digital information is ultimately discrete in nature, lossless compression methods typically proceed from an assumption that their input is a sequence of discrete tokens.
While continuous-valued datasets are still discrete in the sense of being encoded as finite, binary strings, general purpose lossless compression methods often perform poorly due to the lack of readily discoverable statistical structure in this binary space.
Empirically,~\citet{sdrbench_2020} find compression ratios (the ratio of the original data size to the compressed size) of less than 3 for a range of lossless compression algorithms~\citep{zstd, zfpy_2014, fpc_2009, blosc, fpzip_2006} applied to continuous-valued scientific datasets. For many research budgets, compressing a 100 PB atmospheric trajectory ensemble to 33 PB would not meaningfully address data storage challenges.

For the output physical simulations,~\cite{simfs_girolamo_2019} propose to store trajectories as a sparse set of checkpoint frames spaced at regular time intervals, and re-simulate the discarded frames from the nearest preceding checkpoint. The compression ratio is dependent on the frame spacing, and re-simulation may incur significant computational cost. The methods we describe do not assume the existence of, or access to, the original data simulator.

Lossy compression methods, by contrast, allow for some distortion in the recovered signal after decompression.
There exists an inherent tension between the amount of compression (the obtained code's \emph{rate}) and the degree of distortion incurred, the \emph{rate-distortion trade-off}.
The kind and degree of distortion acceptable depends heavily on the application domain, and the quantification and mitigation of application-relevant distortion is central to the design of compression methods.
Domain knowledge also allows the algorithm designer to exploit known statistical regularities in the data to achieve higher compression at a fixed distortion level.

Several error-bounded lossy compression algorithms have been designed for floating-point arrays \citep{sz3_algo,sz3_framework,zfpy_2014,tthresh_2020,sperr_2023}. Among those, we evaluate SZ3~\citep{sz3_algo,sz3_framework} and ZFP~\citep{zfpy_2014} and show in Section \ref{sx:discuss:error-bound} that these methods only achieve approximately $50\times$ compression.
\citet{klower2021compressing}~proposes using lower-precision numbers to represent atmospheric states, effectively discretizing floating-point numbers by rounding them. This achieves compression ratios of up to 155 for temperature, at $\pm 0.4^\circ$~C median error. Neural network-based approaches for compression, that we describe further in the next section, have also recently been introduced by \citet{huang2022compressing} and \citet{han2024cra5}. 

%Greater compression is possible when we can exploit the statistical regularities in the data, suggesting that far greater compression would be possible if we could use machine learning to train a compressor specifically for atmospheric data. When compared to the general-purpose compressors discussed above, we will find that the learned compressors we develop achieve comparable errors while providing a  $1000 \times$ compression.

Our overall approach is best understood within the paradigm of \emph{transform coding}~\citep{goyal2001theoretical}, which underpins most modern methods for the compression of natural signals such as images, audio and video.
In transform coding, the original signal is invertibly mapped into an alternative domain judged more suitable for lossy scalar quantization (for example, certain elements of the transformed representation are known to be less crucial to perceived quality for the reconstruction~\citep{wallace1992jpeg}), and a stream of bits representing indices in the reduced set of quantized scalars is losslessly compressed via entropy coding.
The invertible transform is typically linear (e.g., the familiar JPEG format uses a discrete cosine transform on small square sub-regions), and designed to produce a collection of relatively uncorrelated scalars.
Traditionally, the transform, quantization and entropy coding steps form wholly separate subsystems of a compression pipeline.
While this modularity affords implementation benefits, recent advances in machine learning have demonstrated that quantization can be directly and fruitfully incorporated into scalable representation learning systems.
In this work, we explore two such families of methods, the latter of which also employs a relaxation of the entropy coding objective to directly parameterize the rate-distortion trade-off.

\subsection{Neural Compression}
\label{sx:methods:networks}

The methods explored in this work build upon the \emph{autoencoder} family~\citep{ackley1985learning,hinton1990connectionist} wherein a parameterized non-linear mapping (i.e.\ neural network, best thought of as the composition of an ``encoder'' and a ``decoder'' function) is fit to data, with the goal of the system reproducing its own input from an alternative representation; Figure \ref{fig:system} depicts the overall setup.
Given that the identity function is otherwise trivially representable, constraints imposed on the functional form of an autoencoder (such as a low-dimensional ``bottleneck'' between encoder and decoder, or penalties imposed during optimization) guide the learning procedure in the direction of descriptive parsimony~\citep{elman1988learning,Cottrell1987}.
Probabilistically motivated variants of autoencoders have seen wide use in learning low-dimensional representations of data, and have an established connection to compression theory, formalized in several ways through the minimum description length principle and bits-back-encoding~\citep{hinton1993autoencoders, grunwald2007minimum}, variational inference~\citep{rezende2014reparameterizationtrick,kingma2014vae}.

In contrast to autoencoders, a recent line of work uses neural networks to represent continuous data directly, mapping spatial coordinates to their corresponding data values~\citep{dupont2022functa, xie2022neural_fields_beyond}. For example, the pixels of a single photograph can be used as a ``dataset'' from which to train a network to map pixel coordinates $(i, j)$ to the corresponding pixel color $(r, g, b)$. Once trained, the network's parameters serve as the compressed representation, and can be significantly more compact than the raw array of data they encode.
\citet{huang2022compressing} demonstrate this on atmospheric data on a wide range of compression ratios, but this approach has the disadvantage that it requires training or fine-tuning the model for each new data point (although we note that there are now methods that use meta-learning to address this limitation \citep{coinplusplus_2022}).

%This approach was initially developed for 3D scenes~\citep{mildenhall2020nerf} and has since been extended to other domains such as images and atmospheric states \citep{strumpler2022inrcompress, dupont2021coin,, kim2024hybrid}. \citet{coinplusplus_2022} removes the need to retrain a network from scratch for each new data point, by meta-learning a network for all data, and efficiently fine-tuning it to fit novel datapoints using modulations to its parameters.



%Neural compression models take advantage of the ability of deep neural networks to learn efficient representations of data. Of the many types of neural network architectures, 

%One of the strengths of neural network models is their capacity for learning representations of data \citep{lecun2015deep}, which enables generalisation \citep{lecun1989generalization} and which is often achieved by encoding inputs into sparse \citep{ranzato2007sparse} or low-dimensional representations. Autoencoder networks \citep{hinton1993autoencoders} and their variational versions \citep{rezende2014reparameterizationtrick,kingma2014vae} are a perfect example of learning a compressed representation of input data that can still reconstruct that data. The optimisation of these networks given data is a case of the Minimum Description Length principle  By consequence, autoencoders are an ideal choice for data compression. 
%
%We therefore train a neural network to map data to a compressed representation. This avoids having to train or fine-tune a network for each new data point, unlike in \citep{huang2022compressing}. 
In an autoencoder, the encoder maps rich high-dimensional signals to lower-dimensional codes more suitable for storage or transmission, which can be lossily reconstructed by applying the decoder.
The encoder-decoder framework has several advantages. Once trained, the encoder can be applied to data beyond its training set. The compressed representation can be designed to have the same spatial layout and topology as the input data, aiding interpretability. Of particular interest are strategies for learning \emph{discrete} representations with autoencoders, which lossless compression, and may facilitate direct, downstream use with sequence models such as transformers~\citep{vaswani2017transformer, nguyen2023climax}.
We next describe several families of such autoencoders which achieve discrete representations using two different strategies.
%and describe the architectural details in Appendix~\ref{sx:appendix:models}.

% ---------

% Use of spherical harmonics: "Spherical Fourier Neural Operators: Learning Stable Dynamics on the Sphere" \citep{bonev2023spherical}

% While lossless compression allows to store data without loss of information, \cite{sdrbench_2020} find that lossless compressors such as~\citep{zstd,zfpy_2014,fpc_2009,blosc,fpzip_2006} produce low compression ratios, below 3, on a range of scientific 32-bit floating-point datasets.


% \cite{simfs_girolamo_2019} propose to store checkpoints at regular time steps and re-simulate discarded data for missing steps from the closest saved results.
% This method offers an explicit computation / storage trade-off by adjusting the time step between checkpoints.
% It is also lossless, as simulations can be run to regenerate the discarded time steps.

% \cite{nguyen2023climax}
% \cite{klower2021compressing}
% \cite{coinplusplus_2022} 

% A recent line of work relies to coordinate-based neural networks to compress datasets.
% These networks are optimized to map data coordinates to target signal values for each data sample~\cite{xie2022neural_fields_beyond}.
% The stored neural network weights can be used at decompression time to predict the values of the original sample.
% This approach has been initially developped for 3D scenes~\cite{mildenhall2020nerf} and has since been extended to other domains such as images~\cite{dupont2021coin,strumpler2022inrcompress} and atmospheric states \cite{dupont2021coin,huang2022compressing}.
% Coordinate-based neural networks take numerical coordinates as input and have therefore the advantage to not be restricted to a specific grid resolution.
% However, compared to traditional compression methods, optimizing a neural network for each sample is significantly slower and is therefore not practical for online compression of simulator outputs. \yhasson{Is that true ?}.
% \cite{coinplusplus_2022} reduce fitting requirements at test time by learning a shared network across datapoints and storing modulations which can be computed using a few gradient steps for each sample.
% \cite{tack2023learning} also proposes to speed-up neural network fitting by first learning a shared model, but only computes PSNR, no direct downstream use in compression.

% \cite{kim2024hybrid} propose a hybrid representation of spherical data and compare compression results to \cite{huang2022compressing}.
% They compress each time step separately and achieve slightly higher weighted RMSE and weights MAE errors for similar bits per pixel compared to~\cite{hoefler2023earth}, which compress the data in the temporal dimension as well.

% Compression listed as key component of Earth Virtualization Engines (EVE) \cite{hoefler2023earth}.



==> 03_method.tex <==
\subsubsection{VQ-VAE and VQ-GAN}

The vector-quantized variational autoencoder, or VQ-VAE~\citep{oord2017vqvae} is a neural network that maps input data to a set of discrete indices into a learned codebook of vector-valued codes.
Taking inspiration from \cite{kingma2014vae}, a continuous neural encoder maps the input $x$ to a continuous code layer. While the original VAE relied on amortized inference (by the encoder) of sufficient statistics of continuous random variables and a ``reparameterization trick'' to obtain differentiable samples~\citep{williams1992simple,rezende2014reparameterizationtrick}, the VQ-VAE defines a degenerate variational posterior in which (components of) the latent representation adopt the closest (in Euclidean distance) of $N$ distinct values from a learned codebook~$D$.
In the case of images, convolutional architectures~\citep{lecun1989generalization} are employed for the encoder and decoder, and a vector $z_{ij}$ at each spatial location in the lower dimensional, final layer spatial map is quantized to values from a codebook shared across all spatial locations. The encoder and decoder are trained end-to-end by minimizing the L2 norm between the input data and their reconstructions. During this optimization, the gradients through the non-differentiable quantizing operation are estimated by simply ignoring it and substituting the identity function~\citep{hinton2012coursera,bengio2013estimating,theis2017lossy}.
Additional loss functions steer the codebook entries toward the output of the encoder while also encouraging the encoder to ``pick'' between codebook entries rather than predict convex combinations thereof (see \citet{oord2017vqvae} for details).
%Like a VAE~\citep{kingma2014vae}, it uses a continuous neural encoder to map the input $x$ to continuous-valued means~$\sigma$ and variances~$\mu$ of a set of independent scalar normal distributions. The decoder samples from these distributions to get a latent vector~$z$, which it then feeds through a decoder network to generate an approximation of the input $x'$. The encoder-decoder pipeline is trained end-to-end by stochastically optimizing the MSE reconstruction loss $||x-x'||$. The loss gradients are pushed through the otherwise undifferentiable stochastic sampling step using the ``reparameterization trick''~\citep{kingma2014vae, rezende2014reparameterizationtrick}. This decomposes the sampling step into a differentiable transform and a stochastic noise function with zero mean and unit variance, the latter of which is taken to have no effect on the gradient (in expectation) and is therefore ignored during differentiation. 

%VQ-VAE adds vector quantization to this. Rather than let latent vector~$z$ adopt any value, it constrains it to be one of $N$ possible values from a learned codebook~$D$. 
Once quantized, an encoded value can be parsimoniously represented as an integer index $i \in [1, N]$ such that $z \approx D_i$.
Beyond the compression that results from replacing a multi-channel image with a much smaller array of integers, the resulting map can be further compressed with standard entropy-coding techniques, potentially exploiting both non-uniformity of codebook usage and spatial correlations in the resulting low-dimensional maps. Figure~\ref{fig:vqvae} illustrates the VQ-VAE network, depicting the encoder/decoder and the codebook reconstruction.

As noted in section~\ref{sx:introduction}, na\"ively optimizing the mean squared error can have unacceptable consequences for atmospheric states, as its tendency to wash out sharp features can erase the very events climate scientists wish to measure, such as hurricanes.
We therefore also investigate VQ-GANs~\citep{esser2021taming}, which augment a VQ-VAE by adding a patch-wise discriminator~\citep{isola2017image} and are trained with an auxiliary adversarial loss term~\citep{goodfellow2014gan}. During training, the discriminator receives the quantized feature map indices, channel-wise concatenated (after upsampling and continuous embedding) with either the original atmospheric data from which it was computed or its corresponding reconstruction. The discriminator is trained to maximize its classification accuracy on discriminating patches of real data from reconstruction patches, while the encoder-decoder pipeline is trained to reconstruct its input well while minimizing this accuracy.
Adversarial losses were similarly used for restoring high spatial frequencies for precipitation nowcasting in~\cite{ravuri2021nowcasting}.
For both VQ-VAE and VQ-GAN experiments, we base our neural network architectures on those presented in \cite{esser2021taming}.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/networks/vqgan.pdf}
    \caption{The VQ-GAN network, which contains a VQ-VAE network and an auxiliary discriminator. The encoder and decoder are residual convnets with attention, which reduce the input data into an 18x18 grid of vectors of size 1024. These are then quantized to their nearest match in the learned codebook of N vectors. See Appendix~\ref{sx:appendix:models} for details.}
    \label{fig:vqvae}
\end{figure}

\subsubsection{Factorized prior and Hyperprior Models}

Whereas VQ models discretize a latent vector $z$ to its nearest neighbor in a learned codebook, the factorized prior model~\citep{balle2017fp} discretizes individual elements of $z$ by rounding to integers at test time.
This is approximated during training as a zero-mean scalar noising function in the same spirit as the ``reparameterization trick'' described above.
Unlike the VQ models described earlier, the factorized prior's objective function is explicitly derived with data compression in mind, and a continuous relaxation of the Shannon entropy of the resulting discrete code comprises an additional loss term.
Probabilistically speaking, the encoder-decoder pair are trained to optimize a variational lower bound on the expected log-likelihood of the data modeled by latent variables with a prior consisting of independent uniform random variables (hence, ``factorized'') and an isotropic Gaussian likelihood.
%This noise function is also sampled from during decoding, to convert integers to continuous values.

The hyperprior model~\citep{balle2018hp} is an extension which, for training purposes, composes two factorized prior autoencoders.
The first block's encoder produces a feature map~$z$, which is quantized to integers~$\hat z$.
As is common in convolutional feature maps, the pixels of~$\hat{z}$ retain local spatial correlations.
The second autoencoder implements, with the same variational approach (though a different likelihood function) a probabilistic generative model which captures these correlations, introducing a new, smaller set of latent variables $w$\footnote{\citet{balle2018hp} uses the notation $y$ and $z$, rather than $z$ and $w$, for first and second level latent variables, respectively.}.
The probabilistic model defined by this secondary autoencoder is used to more effectively entropy code the first model's quantized maps $\hat{z}$ by predicting the scale (i.e.\ modeling the variance) of each element of $\hat{z}$ conditioned on the encoded, quantized secondary latent variables $\hat{w}$, which are themselves entropy-coded and stored alongside the  resulting encodings of $\hat{z}$.
Figure~\ref{fig:hyperprior} shows the network schematic for the hyperprior model, while Figure~\ref{fig:balle} gives a detailed picture including layer sizes.
We recommend the hyperprior model as the most suitable neural compressor that performs well across all the key requirements considered in the introduction.

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/networks/hyperprior_horizontal.pdf}
    \caption{Hyperprior network. This augments the factorized prior network (dashed rectangle) by adding an additional encoder-decoder pathway that encodes the FP network's latents, and decodes them to a grid of variances.}
    \label{fig:hyperprior}
\end{figure}



\subsubsection{Effective compression ratio}

The na\"ive compression ratio for the VQ-VAE or VQ-GAN model would consist in dividing the storage space needed for representing input data (e.g., 5 vertical variables times $256 \times 256$ pixels of 32-bit floating point data) vs. the storage space needed by the compressed vector-quantized maps (e.g., for a VQ-VAE with 3 downsampling blocks, $32 \times 32$ indices of a 13-bit dictionary with $2^{13} = 8192$ elements)\footnote{Given that we use overset HEALPix grids detailed in Appendix \ref{sx:appendix:overset_healpix}, the compression is computed as a ratio between $288 \times 288$ 5-channel 32-bit images and $n$-bit $36 \times 36$ maps.}. For this specific example, the compression ratio is about 788. In entropy coding can further reduce the storage footprint, we estimate the compression ratio to be approximately $1100\times$ for that model architecture when compressing test data.

For the purpose of this work, we estimate storage cost in bits as the empirical Shannon entropy of codebook indices per grid, $H = -\sum_i f_i \log_2 f_i$, where $f_i$ is the observed frequency of codebook element $i$ in a given grid. 
This notably ignores expected spatial correlations in the encoded representation (for which the hyperprior model explicitly accounts). The obtained compression ratios for VQ models could thus be improved by fitting a secondary autoregressive model on the codebook index maps\footnote{While not chiefly concerned with compression, \cite{oord2017vqvae} employ autoregressive PixelCNN models of codebook indices to lower-bound the log likelihood of test data as well as for the generation of \emph{de novo} samples.}. The compression ratios obtained with this simplistic entropy computation thus serve as a conservative lower bound.

\subsection{HEALPix map projection}

The representation and projection of the initial data that is to be compressed is a key consideration in the design of neural compression methods, and it is this first step depicted in Figure \ref{fig:system} that we now describe. 
Atmospheric data lies on a sphere, whereas numerical programming natively operates on rectilinear arrays. 
The equirectangular latitude/longitude projection suffers from fundamental limitations in that pixels do not represent consistent units of area across the map, ranging from $28~\text{km} \times 28~\text{km}$ at the equator to negligible area at either pole (where the grid heavily oversamples).
To address these limitations, there exist a multitude of alternative gridding conventions, with the most common reprojections being octahedral~\citep{smolarkiewicz2016fvm} and icosahedral~\citep{zangl2015icon} sampling, cubed spheres~\citep{lin1997cubedsphere,ronchi1996cubed}, dual lat-lon / ``Yin-Yang''~\citep{cote1998gem,ohno2009visualization} maps, and locally linear projections~\citep{metoffice2016data}.

%One workaround to this mismatch is to convert the data to spherical harmonics, a natural means of representing spherical data in a linear array of coefficients. However, reconstruction errors in these coefficients can introduce systematic artefacts across the globe. Unlike convolution-based neural networks, which are geared to encoding local features, spherical harmonics do not represent local features. Another way to avoid projections is to use a model that can represent spherical inputs as a local graph, such as GraphNets~\citep{lam2023graphcast}. However, in our context of compressing a dataset for general use, we prefer to be versatile in the choice of model, many of which use some form of reprojection from the earth's sphere to a two-dimensional array.

% From Table 3 in https://gmd.copernicus.org/preprints/gmd-2017-108/gmd-2017-108-manuscript-version6.pdf

%Researchers often jointly design their models and reprojection schemes, resulting in almost as many gridding conventions as there are models~\citep{ullrich2017review}. These include 
%HEALPix provides three key features not provided by other projections: (1) it is efficiently convertible to any arbitrary other projection and this maintains compatibility with other projections that maybe needed; (2) it naturally splits the data into grids that are of a manageable size for machine learning accelerators such as GPUs and TPUs; (3) it roughly preserves area, thus avoids the need to learn redundant features over multiple scales. %
The Hierarchical Equal Area iso-Latitude Pixelation (HEALPix) projection~\citep{gorski1999healpix} defines a curvilinear partitioning of the sphere into 12 equal-area base pixels, further subdivided by powers of 2 into a local square coordinate system, which can be sized to the needs of the application.
The pixels of a HEALPix grid, when traversed diagonally, lie along lines of constant latitude, making conversion to and from spherical harmonics especially efficient\footnote{We have explored the use of cubed sphere \citep{ronchi1996cubed,lin1997cubedsphere} and Yin-Yang \citep{cote1998gem,ohno2009visualization} projections, that have the advantage of \emph{overset}, i.e., overlapping grids, but where grid points do not lie on equally spaced equilatitude rings that prove useful for the computation of spherical harmonics.}.
This ease of conversion to the lingua franca of spherically embedded continuous data makes HEALPix a convenient grid format for conversion to any other grid format.
HEALPix is widely used in astronomy for data situated on the celestial sphere, and is seeing increasing use in atmospheric science in classical NWP models~\citep{karlbauer2023advancing} and in deep learning-based methods~\citep{ramavajjala2024heal, chang2023seamless}. %, and discussed as a potential standard grid format for the field.

Figure \ref{fig:system} illustrates the projection of atmospheric data onto HEALPix, and specifically shows 3 such HEALPix base pixels (base pixel 7 is equatorial whereas base pixels 10 and 11 are polar). It also illustrates the forward transform of the HEALPix representations to compute spherical harmonics coefficients (analysis), and the inverse transform of spherical harmonics coefficients to compute latitude/longitude projections (synthesis). To avoid losing high-frequency information, we choose maximum wavenumber $l_{max}=721$ (equal to the number of latitudes on the latitude/longitude grid and half the number of longitudes during synthesis of the reprojection image) for the spherical harmonics transform; see Appendix~\ref{sx:appendix:spherical_harmonics} for more details. One important consideration when using HEALPix is that the round-trip from latitude/longitude representations to HEALPix projections at our chosen resolution to spherical harmonic coefficients back to latitude/longitude reprojection introduces small interpolation errors, which remove some high-frequency information (as visible in Figure~\ref{fig:spectra}, illustrating the comparison between power spectra of the ground truth and power spectra of the reprojection).

In the experimental analysis that follows, we will use HEALPix with a $256 \times 256$ pixel grid within each of the 12 top-level base pixels, preserving a spatial resolution of around 0.25 degrees per pixel. For reference, the equirectangular projection in which ERA5 data are distributed contains arrays of 721 latitudes by 1440 longitudes, i.e., $1,038,240$ pixels (with significant oversampling at the poles) whereas the HEALPix projection at $256 \times 256$ contains $786,432$ pixels; we show in Appendix \ref{sx:appendix:overset_healpix} that these HEALPix pixels cover smaller areas than lat/lon cells at the equator.
Similarly to \cite{karlbauer2023advancing}, we also extend HEALPix to support overset grids, or grids with overlapping domains at the edges. On each side of each $256 \times 256$ grid, we add a margin of 16 pixels, whose values are interpolated from the neighboring grids with which they overlap. This enables us to remove discontinuities between neighboring grids in the decompressed data, by linearly blending between the two grids' values where they overlap. See Appendix~\ref{sx:appendix:overset_healpix} for details.

%While not focused on data compression but rather on weather forecasting and climate modeling tasks, a number of recent deep learning methods tackled spherical data, from GraphCast \citep{lam2023graphcast} and GenCast \citep{price2023gencast} operating on local Graph Neural Networks, as well as Convolutional Graph Networks \citep{defferrard2019deepsphere} or Spherical Convnets \citep{cohen2018spherical}, to Spherical Fourier Neural Operators \citep{pathak2022fourcastnet,bonev2023spherical}.


==> 04_experiments.tex <==
\section{Results}
\label{sx:experiments}

\subsection{Data and Standardization}
We study the ECMWF ERA5 dataset~\citep{era5} of atmospheric states. This dataset is the result of reanalysis, or fitting a physics simulation to sparse historical data, thereby generating a "movie" of atmospheric state, with values sampled in a dense regular grid over space and time. The frames are sampled hourly from 1 January 1959 to 10 January 2023, resulting in 561,264 frames.

From this dataset we extracted two subsets for study: a surface level dataset and a vertical levels dataset which spans a range of elevations from the surface up to the lower stratosphere. The surface dataset contains four variables: temperature at 2~m, pressure at surface, and the 2D (zonal and meridional) wind velocity at 10~m. The vertical levels are in fact pressure levels, or isosurfaces of constant pressure, and contain five variables for each level: temperature, specific humidity, geopotential, and the 2D wind velocities. 
%As is common practice, the elevation levels are not defined by elevation per se, but rather they are pressure levels, or isosurfaces of constant pressure. 
Of ERA5's full complement of 137 pressure levels, we selected 13, at 50, 100, 150, 200, 250, 300, 400, 500, 600, 700, 850, 925, and 1000~hPa. When represented in uncompressed 32-bit floating point, these two datasets are 6 TB and 97 TB respectively.
We standardize all atmospheric variables to zero mean, unit standard deviation per pressure level based on the mean and standard deviation computed across all frames of the training dataset.

\subsection{Train/test split and generalisation}

In order to assess the generalization capabilities of our models, we split the data into a training set spanning 1 January 1959 through 31 December 2009, representing 447,072 frames over 51 years, and a test set spanning 1 January 2010 through 10 January 2023, representing 114,192 frames over slightly more than 13 years. Section \ref{sx:discuss:generalisation} investigates if and how reconstruction error deteriorates as a function of time across the test set.
%
When comparing to the baseline method \citep{huang2022compressing}, we use the dates and timestamps of their ``Dataset 2'', namely 366 frames at midnight of each day in 2016.

\subsubsection{Conditioning on side information}

As terrain features have significant impact on the evolution of atmospheric state, we hypothesized that performance could be improved by augmenting the model with orographic information.
In addition to the atmospheric variables being compressed, the encoder is provided with 6 additional channels of information, corresponding to: the logarithm of the elevation in meters plus 1~m (where elevation had been cropped to be between 0 and 8850~m); the binary land/sea mask, the cosine and sine of the colatitude in radians; the cosine and sine of the longitude in radians. We obtained elevation data from the Google Earth Engine, accessing the GTOPO30 Global 30 Arc-Second Elevation from USGS (at about 1km resolution)\footnote{\url{https://developers.google.com/earth-engine/datasets/catalog/USGS_GTOPO30}}; NaN elevation values correspond to seas: we replace them by 0 for the elevation channel, while also using them to create the second channel with land-sea mask.

Vertical models are trained to reconstruct one pressure level at a time, conditioned on the target vertical level.
We incorporate this information using FiLM layers (feature-wise linear modulation, \citet{perez2018film}) throughout the encoder and decoder.
For simplicity, in these experiments we represent the pressure level as one-hot vector with 13 elements; FiLM at a given layer then corresponds to incorporating a learnable scale and offset per pressure level.

\subsection{Compression Results}

We present experimental support for the following claims:
\begin{enumerate}
    \item We achieve compression ratios of $1000\times$ and above while keeping the mean absolute error (MAE) low, around 0.4$^\circ$~K (for temperature), around 0.5 $\text{m}/\text{s}$ (for zonal and meridional wind), below 1 hPa for surface pressure and around 50 $\text{m}^2/\text{s}^2$ for geopotential.
    \label{claim:cr_and_mae}
    \item Only a small number of reconstructed pixels exhibit errors that exceed given thresholds: about 0.5\% pixels beyond 1$^\circ$~K error in temperature, about 0.5\% pixels beyond 1 $\text{m}/\text{s}$ error in zonal and meridional wind, about 0.15\% pixels beyond 1 hPa error in surface pressure, and about 0.05\% pixels beyond 100 $\text{m}^2/\text{s}^2$ error in geopotential. \label{claim:few_bad_pixels}
    \item Our spectral error is kept low, preserving most high-frequency features in the reconstruction images.
    \item We preserve rare and extreme events such as hurricanes and heat waves.
\end{enumerate}
%
Below we evaluate a number of models, described in section~\ref{sx:methods:networks}. Of these, the hyperprior model trained with rate-distortion penalty coefficient 0.025 achieved a compression ratio of around $1000 \times$ while satisfying all of the above claims, in particular preserving the spectral error over most spatial scales. For comparison, we also exhibit the VQ-VAE with 3 downsampling blocks, which outputs $36 \times 36$ VQ maps of 13-bit (or 8192-element) indices into a learned codebook of quantized vectors; that VQ-VAE model achieves a compression ratio $1100 \times$. We observe that the VQ-GAN architecture with similar VQ code dictionary size and number of layers performed similarly to VQ-VAE, which is why we focus only on the VQ-VAE in the analysis.
Finally, we compare these models with a VQ-VAE with 4 downsampling blocks trained exclusively to reconstruct one single variable (geopotential), with a compression ratio of $1800 \times$, and we discuss the advantages and drawbacks of single-channel compressors.


\subsection{High compression ratio with low RMSE \& MAE}

We first define the metrics and notation used in the results. Following the notation of \cite{lam2023graphcast}, we define $D_{\text{eval}}$ as the set of evaluation dates and timestamps, $G_h$ as the grid of $256 \times 256$ pixels in HEALPix tile $h$, while $x_{j,i}$ and $\hat x_{j,i}$ respectively are the ground truth and the reconstruction at the $i$-th pixel of a grid at the $j$-th variable and pressure level. Equations \ref{eq:mae} and \ref{eq:rmse} describe the MAE and RMSE metrics we use for HEALPix projection results.

\begin{equation}
    \text{MAE} (j) = \frac{1}{12 \times | D_{\text{eval}} |} \sum _{d \in D_{\text{eval}}, 0 \leq h \leq 11} \frac{1}{| G_h |} \sum _{i \in G_h} | x_{j,i} - \hat x_{j,i} |
    \label{eq:mae}
\end{equation}

\begin{equation}
    \text{RMSE} (j) = \frac{1}{12 \times | D_{\text{eval}} |} \sum _{d \in D_{\text{eval}}, 0 \leq h \leq 11} \sqrt{\frac{1}{| G_h |} \sum _{i \in G_h} || x_{j,i} - \hat x_{j,i} ||_2^2}
    \label{eq:rmse}
\end{equation}

On the re-projected latitude/longitude grid $G_{0.25^\circ}$ of cells spaced by $0.25^\circ$, we define weighted MAE (Eq. \ref{eq:weighted_mae}) and weighted RMSE (Eq. \ref{eq:weighted_rmse}) as weighted by coefficient $a_i$ which is proportional to the area of the latitude/longitude cell (i.e., to the cosine of the colatitude of the $i$-th cell of latitude/longitude grid) and normalized to sum to 1 over the grid. We also define the traditional weighted RMSE, used by \citet{huang2022compressing}, in Equation \ref{eq:weighted_rmse_trad}.

\begin{equation}
    \text{wMAE} (j) = \frac{1}{| D_{\text{eval}} |} \sum _{d \in D_{\text{eval}}} \frac{1}{| G_h |} \sum _{i \in G_{0.25^\circ}} a_i | x_{j,i} - \hat x_{j,i} |
    \label{eq:weighted_mae}
\end{equation}

\begin{equation}
    \text{wRMSE} (j) = \frac{1}{| D_{\text{eval}} |} \sum _{d \in D_{\text{eval}}} \sqrt{\frac{1}{| G_{0.25^\circ} |} \sum _{i \in G_h} a_i || x_{j,i} - \hat x_{j,i} ||_2^2}
    \label{eq:weighted_rmse}
\end{equation}

\begin{equation}
    \text{wRMSE}_{\text{trad}} (j) = \sqrt{\frac{1}{| D_{\text{eval}} |} \sum _{d \in D_{\text{eval}}} \frac{1}{| G_{0.25^\circ} |} \sum _{i \in G_h} a_i || x_{j,i} - \hat x_{j,i} ||_2^2}
    \label{eq:weighted_rmse_trad}
\end{equation}


Figure~\ref{fig:reprojection_error_vs_cr} shows the reconstruction results evaluated in latitude/longitude projection, namely the RMSE, the MAE and the 0.99999 quantile of error for several models. For our target compression ratio of $1000 \times$, we find the hyperprior model to be the strongest performer. Additionally, Figures \ref{fig:error_vs_cr} in the Appendix provides results in HEALPix projection, comparing the various models both on surface and vertical data reconstruction at multiple levels.   

\subsection{Small number of erroneous pixels in reconstructions}
\label{sx:experiments:bad-pixels}

Figure~\ref{fig:error_histograms} presents a histogram with the distribution of absolute pixelwise reconstruction errors over the entire evaluation set, for three of the vertical variables (temperature, geopotential and zonal wind) and for each elevation level (colour-coded from 50 hPa in blue to 1000 hPa in red). On the top row, corresponding to the hyperprior model, the distributions show sparse tails, with few pixels (0.01\%) reaching high errors of $\pm 4^\circ$~K, $\pm 400~\text{m}^2/\text{s}^2$ or $\pm 6~\text{m}/\text{s}$.

Tables~\ref{tab:percent_bad_pixels_hyper} (for the hyperprior model) and Table \ref{tab:percent_bad_cells_vqvae} (for the VQ-VAE with 3 downsampling blocks) quantify these ``bad pixels'', showing that only 0.5\% pixels at most have absolute errors exceeding 1$^\circ$~K (temperature) or 1 $\text{m}/\text{s}$ (zonal and meridional wind speeds) across all pressure levels.

Because only a few pixels exceed this maximum error threshold, we can trivially cap the maximum error by storing the original uncompressed values of these ``bad pixels'' in a list, to be stored alongside the compressed representation. When reconstructing the image, we overwrite the bad pixels using their original values, reducing their reconstruction error to zero, and capping the maximum error over all reconstructions. The sparsity of bad pixels limits the size of this list, keeping the overall compression ratio low even after accounting for the list's storage cost. The trade-offs of the different strategies for storing this auxiliary information, in terms of compression ratio and distortion characteristics, require further study.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.32\textwidth, trim = 0cm 0cm 1cm 0cm, clip]{figures/experiments/quantiles/errors_Hyperprior_temperature.pdf}
    \includegraphics[width=0.32\textwidth, trim = 0cm 0cm 1cm 0cm, clip]{figures/experiments/quantiles/errors_Hyperprior_geopotential.pdf}
    \includegraphics[width=0.32\textwidth, trim = 0cm 0cm 1cm 0cm, clip]{figures/experiments/quantiles/errors_Hyperprior_u_component_of_wind.pdf}
    \includegraphics[width=0.32\textwidth, trim = 0cm 0cm 1cm 0cm, clip]{figures/experiments/quantiles/errors_3-VQ-VAE_temperature.pdf}
    \includegraphics[width=0.32\textwidth, trim = 0cm 0cm 1cm 0cm, clip]{figures/experiments/quantiles/errors_3-VQ-VAE_geopotential.pdf}
    \includegraphics[width=0.32\textwidth, trim = 0cm 0cm 1cm 0cm, clip]{figures/experiments/quantiles/errors_3-VQ-VAE_u_component_of_wind.pdf}
    \caption{Distribution of signed errors, with the error in the variable units on the X axis and the fraction of pixels in the evaluation set (2010-2023) at that error levels. Top row shows hyperprior results, bottom row shows 3-block VQ-VAE results, with columns corresponding to temperature, geopotential and zonal wind speed. On each plot we show coloured curves for each of the 13 levels in the vertical dataset.}
    \label{fig:error_histograms}
\end{figure}

\begin{table}[]
    \centering
    \caption{Fraction of pixels with absolute error exceeding given error thresholds, for the hyperprior model with about $1000 \times$ compression ratio.}
    \begin{tabular}{c|c|c|c}
        Variable & Error thresh. &\% bad pixels & Compression ratio \\
        \hline
        % Temp \@ 2 m &  \todo{X}$^\circ$~K & \todo{Y\%} & \todo{1000} & \todo{500} \\
        % Surface pressure & \todo{X} hPa & \todo{Y\%} & \todo{1000} & \todo{500} \\
        % Zonal wind & \todo{X} $\text{m}/\text{s}$ & \todo{Y\%} & \todo{1000} & \todo{500} \\
        % Meridional wind & \todo{X} $\text{m}/\text{s}$ & \todo{Y\%} & \todo{1000} & \todo{500}
        Temperature (all levels) & 1$^\circ$~K & 0.5\% & $1059 \times$ \\
        Zonal wind (all levels) & 1 $\text{m}/\text{s}$ & 0.5\% & $1059 \times$ \\
        Meridional wind (all levels) & 1 $\text{m}/\text{s}$ & 0.5\% & $1059 \times$ \\
        Geopotential (all levels) & 100 $\text{m}^2/\text{s}^2$ & 0.05\% & $1059 \times$ \\
    \end{tabular}
    
    \label{tab:percent_bad_pixels_hyper}
\end{table}

\begin{table}[]
    \centering
    \caption{Fraction of pixels with absolute error exceeding given error thresholds, for the 3-block VQ-VAE model with $1100 \times$ compression ratio, and for the 4-block VQ-VAE model with $1800 \times$ compression ratio trained only on geopotential (last row).}
    \begin{tabular}{c|c|c|c}
        Variable & Error thresh. & \% bad pixels & Compression ratio \\
        \hline
        % Temp \@ 2 m &  \todo{X}$^\circ$~K & \todo{Y\%} & \todo{1000} & \todo{500} \\
        % Surface pressure & \todo{X} hPa & \todo{Y\%} & \todo{1000} & \todo{500} \\
        % Zonal wind & \todo{X} $\text{m}/\text{s}$ & \todo{Y\%} & \todo{1000} & \todo{500} \\
        % Meridional wind & \todo{X} $\text{m}/\text{s}$ & \todo{Y\%} & \todo{1000} & \todo{500}
        Temperature (all levels) & 1$^\circ$~K & 0.52\% & $1110 \times$ \\
        Zonal wind (all levels) & 1 $\text{m}/\text{s}$ & 0.51\% & $1110 \times$ \\
        Meridional wind (all levels) & 1 $\text{m}/\text{s}$ & 0.51\% & $1110 \times$ \\
        Geopotential (all levels) & 100 $\text{m}^2/\text{s}^2$ & 0.063\% & $1110 \times$ \\
        \hline
        Geopotential$^*$ (all levels) & 100 $\text{m}^2/\text{s}^2$ & 0.012\% & $1796 \times$ \\
    \end{tabular}
    
    \label{tab:percent_bad_cells_vqvae}
\end{table}


\subsection{Spectral properties of the reconstructions}

Figure~\ref{fig:spectra} shows the power spectrum density for 4 of the reconstructed variables (temperature, specific humidity, zonal wind and geopotential), with spectra averaged over all equirectangular latitude/longitude frames and over all vertical levels. We notice that some high-frequency information is automatically lost after a round-trip consisting of HEALPix projection from latitude/longitude, spherical harmonic analysis of HEALPix tiles and spherical harmonic synthesis from the spherical harmonics coefficients.

Figure~\ref{fig:spectra} shows that the spectrum of hyperprior reconstructions is closest to the spectrum of ground truth than that of 3-block VQ-VAEs for all variables.
Appendix~\ref{sx:appendix:spherical_harmonics} details the computation of spherical harmonics on HEALPix tiles, and the extraction of the power spectral density from spherical harmonics coefficients.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth, trim = 5cm 0cm 5cm 0cm, clip]{figures/experiments/spectrum/reprojection_spectra.pdf}
    \hfill
    \caption{Power spectrum density for temperature, specific humidity, zonal wind and geopotential, computed using forward spherical harmonics transform. Results are computed on the daily 2016 baseline dataset.}
    \label{fig:spectra}
\end{figure}


\subsection{Extreme values}

In order to more fully understand the behaviour of these models, we manually select dates corresponding to extrema in temperature, such as Indian heatwave of 2015, and to hurricanes, such as Hurricane Harvey in September 2017 and Hurricane Matthew in October 2016. Figures \ref{fig:hurricane_matthew_hyperprior} and \ref{fig:hurricane_matthew_vqvae} illustrate the performance of the hyperprior and 3-block VQ-VAE models on Hurricane Matthew, and show that geopotential and wind speed information corresponding to the eye of the cyclone is preserved after compression and reconstruction. Figure~\ref{fig:heatwave} illustrates the reconstruction of the temperature at 1000 hPa over 24 hours on 23 May during the 2015 Indian heatwave, and shows that temperature extrema up to around $45^\circ~\text{C}$ are correctly represented.

Appendix~\ref{sx:appendix:hist2d-err-value} contains additional analysis of the reconstruction errors, which suggest that the hyperprior compression model errors are roughly uniformly distributed over the target values, and that the model tends to overestimate higher temperature and wind speed and underestimate lower temperature or wind speed.

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth, trim = 6cm 2.5cm 5cm 2cm, clip]{figures/experiments/heatwave/2015_5_23-6_HyperPrior_temperature_zoom_1000hPa.pdf}
    \includegraphics[width=0.9\textwidth, trim = 6cm 2.5cm 5cm 2cm, clip]{figures/experiments/heatwave/2015_5_23-12_HyperPrior_temperature_zoom_1000hPa.pdf}
    \includegraphics[width=0.9\textwidth, trim = 6cm 2.5cm 5cm 2cm, clip]{figures/experiments/heatwave/2015_5_23-18_HyperPrior_temperature_zoom_1000hPa.pdf}
    \includegraphics[width=0.9\textwidth, trim = 6cm 2.5cm 5cm 2cm, clip]{figures/experiments/heatwave/2015_5_24-0_HyperPrior_temperature_zoom_1000hPa.pdf}
    \hfill
    \caption{Reconstructions of temperature at 1000 hPa from 2015/5/23 at 6, 12, 18 and 24 UTC (during the 2015 Indian heatwave). Globally, MAE is about $0.47-0.48^\circ~\text{K}$ and most the area of interest is under $1^\circ~\text{K}$ error. The residual show that a few scattered areas near Bhutan or near Karachi have reconstruction over-estimated by about $2-3~^\circ~\text{K}$.}
    \label{fig:heatwave}
\end{figure}

\subsection{Comparison with baseline method}

To be able to compare results with \cite{huang2022compressing}, we use the same dataset (described in \cite{ashkboos2022ens}) which contains 11 pressure levels, including 10 of ours and one extra pressure level at 10 hPa. Appendix~\ref{sx:appendix:huangiclr2023} explains how we run their code and establish parity between evaluating on their 11 pressure levels and our 13 pressure levels.

We also define the same subset of data (corresponding to Dataset 2 in \citet{huang2022compressing}), namely 366 daily frames (at 0 UTC) in 2016\footnote{Note that results on Figs. \ref{fig:spectra}, \ref{fig:error_vs_cr} and \ref{fig:reprojection_error_vs_cr_bounded_compression} are computed on the reduced subset of 366 daily frames (at 0 UTC) in 2016.}.

In Figure~\ref{fig:error_vs_cr}, our VQ-VAE, VQ-GAN and hyperprior models achieve significantly lower temperature errors (e.g., $\text{MAE}=0.3^\circ$~K for the $1000 \times$ hyperprior model) than the baseline method. For geopotential, our compression results are marginally better than the baseline ($\text{MAE}=45~\text{m}^2/\text{s}^2$ for the $1000 \times$ hyperprior model, vs. $60~\text{m}^2/\text{s}^2$ for the $1300 \times$ baseline).

Two main observations arise: 1) it is worth investigating single-variable compression of geopotential, similarly in the baseline models (see additional results in Section \ref{sx:discuss:geopotential}), and 2) the baseline method can achieve similar if not better error maxima. We discuss error maxima and provide detailed analysis of the possible origin of the errors in Appendix~\ref{sx:appendix:analysis}.

In concurrent work,~\citet{han2024cra5} demonstrate a neural compressor applied to ERA5 in lat-lon format, with a number of important differences from our own work. While we explore both VQ-VAE and hyperprior networks as candidate models, \citet{han2024cra5} propose a stagewise training method based on a single VQ-VAE network incorporating a window-based attention mechanism to encode the data to latent variables, and another to serve as a hyperprior block to encode first-level variances.
They validate and test on 2022 and 2023 data respectively, whereas we train on data up to 2010 and evaluate long-term generalisation on 2010-2023.
They report comparable RMSE to what we report in this work, while that work reports compression ratios of $229-323\times$ compared to the ratios of $1000-3000\times$ that we report.
%\mkg{Should we go into any more detail about ~\citep{han2024cra5} here? We should add a comparison of their RMSE to ours, using the figures from their table 2. If we wish to be rigorous we could run our evaluator only on 2023 data, the way they do.}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth, trim = 6cm 0cm 6.5cm 0cm, clip]{figures/experiments/reprojection_stats/reprojection_weighted_rmse_mae_all_temperature.pdf}
    \includegraphics[width=1\textwidth, trim = 6cm 0cm 6.5cm 0cm, clip]{figures/experiments/reprojection_stats/reprojection_weighted_rmse_mae_all_geopotential.pdf}
    \includegraphics[width=1\textwidth, trim = 6cm 0cm 6.5cm 0cm, clip]{figures/experiments/reprojection_stats/reprojection_weighted_rmse_mae_all_specific_humidity.pdf}
    \includegraphics[width=1\textwidth, trim = 6cm 0cm 6.5cm 0cm, clip]{figures/experiments/reprojection_stats/reprojection_weighted_rmse_mae_all_u_component_of_wind.pdf}
    \hfill
    \caption{Reconstruction and reprojection error vs. compression ratio, for vertical data, in equirectangular projection. Columns: metrics: respectively root mean squared error (RMSE), mean absolute error (MAE), 0.99999 quantile of error and maximum error over the daily 2016 baseline dataset. Lower errors and higher compression rates are better (bottom right of each plot).}
    \label{fig:reprojection_error_vs_cr}
\end{figure}




==> 05_discussion.tex <==
\section{Analysis and Discussion}
\label{sx:discussion}

Next, we motivate the use of neural compression methods by comparison with error-bound compression, discuss the possibility of compressing high-error residuals (Section \ref{sx:discuss:error-bound}), and present results for single-variable models (Section \ref{sx:discuss:geopotential}). A principal limitation of  neural compression methods for scientific data is that they have unbounded (and potentially high) maximum element-wise reconstruction errors. We investigate and explain a cause of this high error for the ERA5 dataset as being due to artefacts present in the dataset as well as joint reconstruction of multiple variables (Section \ref{sx:discuss:limitation-artefacts}). Finally, we evaluate performance of generalization over time in Section \ref{sx:discuss:generalisation}).


\subsection{Comparison with error-bounded compression}
\label{sx:discuss:error-bound}

\begin{figure}
    \centering
    \includegraphics[width=1\textwidth, trim = 3cm 0cm 4cm 0cm, clip]{figures/experiments/reprojection_stats/reprojection_weighted_rmse_mae_bounded_compression_all_temperature.pdf}
    \hfill
    \caption{Reconstruction and reprojection error vs. compression ratio, for vertical data, in equirectangular projection. Columns: metrics: respectively root mean squared error (RMSE), mean absolute error (MAE) and maximum error. Results are computed on the daily 2016 baseline dataset. Lower errors and higher compression rates are better (bottom right of each plot).}
    \label{fig:reprojection_error_vs_cr_bounded_compression}
\end{figure}

Our compression techniques achieve strong compression ratios for comparable mean reconstruction errors compared to conventional and competing methods.
However, they lack the precise error bound guarantees provided by off-the-shelf compression tools. 
To address this, we investigated compressing the residuals post-neural compression using both~\citet{sz3_algo} and~\citet{zfpy_2014} to ensure both compression performance and error control. As shown in Figure \ref{fig:reprojection_error_vs_cr_bounded_compression}, bounded compression methods such as SZ3 achieve far lower compression ratios of temperature (i.e., less than $50\times$) for similar errors (namely, weighted RMSE and weighted MAE of the order of $1^\circ$~K) than the neural compression models.

We compared further compressing the residuals of neural compression (e.g., the hyperprior reconstructions in HEALPix projection minus the ground truth in HEALPix projections) and observed similar compression ratios at given error bounds; in other words, compressing the residual was as expensive as compressing the original data using bounded compression methods. We note that SZ3 operates on 1D data, and as such does not exploit the spatial correlations in the data.

From the results in section~\ref{sx:experiments:bad-pixels}, about $0.5\%$ of reconstructed HEALPix pixels present errors higher than the error threshold of $\pm 1^\circ$~K. We could consider compressing the values of those pixels using the SZ3 bounded compression method at a compression ratio of the order of $10\times$, which would result in the order of $1000\times$ compression ratio. However, we would still need to store the byte position (row and column) of those high-error pixels in the $256 \times 256$ tile, or preferably, develop a storage strategy that exploits local spatial correlations of those erroneous pixels. It is also not obvious that such a method would not create additional discontinuities (and as a consequence, high-frequency artefacts) in the reconstructed images. 

\subsection{Comparison with single-variable models}
\label{sx:discuss:geopotential}

The approach we present is developed for multivariate compression, i.e. compression of multiple atmospheric variables using a single latent code.
It is also possible to develop compression models for individual variables.
Figure \ref{fig:reprojection_error_vs_cr} shows that the 4-block VQ-VAE model trained only on geopotential data manages to reconstruct geopotential with $\text{MAE} = 0.2~\text{m}^2/\text{s}^2$ at all levels latitude/longitudewhile maintaining an effective compression ratio of $1800\times$. The last row of Table \ref{tab:percent_bad_cells_vqvae} highlights that very few (0.012\%) pixels cross the 100 $\text{m}^2/\text{s}^2$ error threshold. The right-most column of Figure \ref{fig:spectra} shows that the power spectrum of that model's reconstructions of geopotential are the closest to the spectrum of the reprojection.

% ---Too much detail for initial tech report---
%While multivariate compression is able to exploit correlations in the data, this single-variable compression result points to a promising alternative for achieving higher compression rates. Although, single-variable neural compression requires running as many models as there are atmospheric variables of interest.
%This finding suggests a potential modular modification of the proposed architecture: compressing multivariate weather data into a single common representation that incorporates context from different physical variables, then reconstructing individual variables separately using dedicated decompressors.


\subsection{Difficulty in learning and reconstructing specific variables and pressure levels}
\label{sx:discuss:limitation-artefacts}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth, trim = 0cm 25.5cm 2cm 3.5cm, clip]{figures/experiments/error_vs_level/rmse_across_levels_variables_Hyperprior.pdf}
    \includegraphics[width=0.45\textwidth, trim = 0cm 25.5cm 2cm 3.5cm, clip]{figures/experiments/error_vs_level/rmse_across_levels_variables_3-VQ-VAE.pdf}
    \hfill
    \caption{Standardised RMSE of different variables and atmospheric levels for a single hyperprior model (left) and a 3-block VQ-VAE model (right) at about $1000\times$ compression ratios.}
    \label{fig:rmse_comparison_variables}
\end{figure}

We investigate which variables and pressure levels pose particular challenges for our models.
Recall that prior to training, individual variables are standardised to zero mean, unit standard deviation per pressure level, with means and standard deviations computed across all frames of the training dataset.
While it is important to ground most analyses in ``unstandardised'' computations such that deviations between reconstruction and ground truth are reported the correct units for each variable, comparing the characteristics of individual reconstructed variables before the standardisation is undone can provide insight into the information being preserved by the encoded representation.
%The surface models take 4 channels representing temperature at 2 m, surface pressure, zonal and meridional wind speeds at 10 m as inputs and as targets for the reconstruction; the vertical models take in and predict 5 channels representing temperature, geopotential, zonal and meridional wind speed, and specific humidity.

Figure \ref{fig:rmse_comparison_variables} depicts the \emph{standardized} average root mean square error computed separately for different variables and different pressure levels, for both the hyperprior model at around $1000\times$ compression rate and the 3-block VQ-VAE model at $1100\times$ compression rate. We first notice that the hyperprior model achieves lower RMSE across all variables than the 3-block VQ-VAE model. We also observe that specific humidity consistently has the lowest RMSE overall among vertical data models, and that surface pressure has the lowest RMSE among surface models; then comes temperature, and then wind speed and geopotential. We observe interesting patterns persistent across models, such as wind speeds at 850 hPa having the highest RMSE.

We notice that the main difference between the RMSE profile for the hyperprior model and the VQ-VAE model is the higher RMSE at 50 hPa. In fact, other deep learning models seem to have faced relatively poor performance at the 50 hPa level when training on the same dataset, as evidenced by the per-pressure level scorecards for the GraphCast model~\citep{lam2023graphcast} (in particular, see Figs. 2 and 29, where the prediction skills is significantly lower than at other pressure levels). We surmise that these reconstruction or prediction errors are due to out-of-sample, low-value anomalies in the specific humidity at 50 hPa, at the limit of the upper part of the troposphere, and present a detailed analysis of the data artefacts in Appendix \ref{sx:appendix:artefacts}.
A potential remedy is to simply extend the training set: while autoencoders can be applied to data beyond the training set, it is entirely valid to train a bespoke compressor and decompressor on an entire target dataset if the performance requirements justify the additional computation.

Figure \ref{fig:error_histograms} seems to suggests that error maxima should be bounded, as the $10^{-5}$ fraction of errors 
corresponds to about $\pm 5^\circ$~K (temperature), $\pm 400~\text{m}^2/\text{s}^2$ (geopotential) or $\pm 8~\text{m}/\text{s}$ (zonal wind speed). However, looking at the error maxima on Figure \ref{fig:reprojection_error_vs_cr} shows that the max errors (over 366 frames of the daily 2016 dataset subset) of the hyperprior are as high as $\pm 18^\circ$~K, $\pm 4000~\text{m}^2/\text{s}^2$ and $\pm 40~\text{m}/\text{s}$. Higher error maxima appear on the full test dataset covering 2010-2023.

Our error analysis exposes three potential shortcomings of autoencoder methods. The first is that these models lack error-bound guarantees.
Second, these methods seem to poorly handle out-of-sample artefacts in the data, which may cause them to produce reconstructions with unbounded errors (see analysis of artefacts in Appendix \ref{sx:appendix:artefacts}). Lastly, while compressing variables jointly fruitfully exploits statistical redundancy across variables, this results in brittleness, where an artefact present in the values of one variable may contaminate the reconstruction of another variable.

%The latter point confirms the conclusion from previous section \ref{sx:discuss:geopotential}. The original design choice to process multiple variables at a time was prompted by exploiting correlations in the weather variables; our current area of investigation is to reconstruct different variables separately, as our preliminary results on the compression of geopotential compression using a 4-block VQ-VAE seem to suggest. 


\subsection{Generalisation of compression over time}
\label{sx:discuss:generalisation}

Unlike methods where the neural network is trained to be a functional over the training data, such as our baseline data compression method \citep{huang2022compressing}, our autoencoder-based approach allows for generalization to unseen data frames; this is a significant advantage as we do not need to retrain the compression model to handle new data frames.

Given that weather and climate processes are not stationary, a pressing question is whether, and how quickly, the compression model deteriorates as a function of time. Our dataset split with training on data covering 1959 through 2009, and evaluation on data covering 2010 through 10 January 2023, allows us to test that hypothesis over 13 years. % and focuses on over a decade of ever-intensifying climate change and global warming.

Figure \ref{fig:generalisation-time} illustrates the absolute value RMSE (averaged over HEALPix squares, hours of the days and days of the month) for 4 variables and 5 different pressure levels, as well as a yearly rolling average. The yearly average of temperature, wind speed and specific humidity at 500 hPa, 850 hPa and 1000 hPa seem to have an upward trend over the years. The simplest explanation for such a trend would be that the model is expected to perform worse on test samples that are further away from the training data cutoff date (in our case, 31 December 2009).

However, the monthly average clearly exhibits strong seasonal tendencies that dominate the variability of the yearly rolling average. The standardized RMSE has similar seasonalities, as does the RMSE of the 3-block VQ-VAE model. We also know that because of the unequal land mass distribution between the northern and southern hemisphere, weather variables such as global temperature exhibit seasonality.% We therefore hypothesize that our neural compression models may be heteroskedastic, meaning that it has reconstruction errors that depend on the measured value. A possible strategy to remedy against this is to include conditioning on the time of the year into the model inputs.

\begin{figure}[tbp]
    \centering
    \includegraphics[width=\textwidth, trim = 5.5cm 0cm 5cm 0cm, clip]{figures/experiments/time/time_Hyperprior_rmse_cropped_level100.pdf}
    \includegraphics[width=\textwidth, trim = 5.5cm 0cm 5cm 0cm, clip]{figures/experiments/time/time_Hyperprior_rmse_cropped_level500.pdf}
    \includegraphics[width=\textwidth, trim = 5.5cm 0cm 5cm 0cm, clip]{figures/experiments/time/time_Hyperprior_rmse_cropped_level850.pdf}
    \includegraphics[width=\textwidth, trim = 5.5cm 0cm 5cm 0cm, clip]{figures/experiments/time/time_Hyperprior_rmse_cropped_level1000.pdf}
    \hfill
    \caption{Plot of the average RMSE over 13 years of the test set, from 1/1/2010 to 31/12/2022, using the hyperprior with about $1000\times$ compression rate. Rows from top to bottom show results at 50 hPa, 100 hPa, 150 hPa, 500 hPa, 850 hPa and 1000 hPa, and columns show temperature, geopotential, zonal wind speed and specific humidity. The blue curve shows the monthly average (and exhibits strong seasonal tendencies); the red dashed curve shows the yearly rolling average (and suggests an upward trend over the years, the further away the test sample from the training data cutoff date of 31 December 2009).}
    \label{fig:generalisation-time}
\end{figure}

==> 06_conclusions.tex <==
\section{Conclusion}
\label{sx:conclusion}

We propose a method for the neural compression of atmospheric states using the area-preserving HEALPix projection to simplify the processing, by conventional neural networks, of data situated on the sphere. We highlight that this choice of projection allows for efficient computation of spherical harmonics, thereby simplifying both the reprojection of decompressed atmospheric states to latitude/longitude coordinates and straightforward interrogation of the spectral properties of the reconstructions.
We conduct a detailed analysis of the performance characteristics of several neural compression methods, demonstrating very high compression ratios in excess of $1000\times$ with minimal distortion, while also drawing attention to several shortcomings.
We find that the hyperprior model, even with a relatively simple encoder and decoder, appears best suited to the task among the models studied.
Notably, the hyperprior model largely preserves the shape of the power spectrum, despite being trained only via mean squared error and a compressibility penalty.
We examine performance of the studied compressors on states representing extreme atmospheric events and find that these, too, are well-preserved.
These results make a compelling case for the viability of neural compression methods in this application domain, while our analysis elucidates trade-offs inherent in our approach, as well as practical considerations surrounding the design of error-bounded compression systems atop these methods.

%Ongoing work focuses on open-sourcing the code and model weights of the hyperprior model, as well as on releasing compressed versions of several climate datasets including (and beyond) ERA5. Because of the representational power of compressed representations, we are also investigating upstream applications of our models for weather and climate forecasting.

%Thanks to careful analysis of the error maxima, we identified the source of high errors in the compression of temperature or geopotential, which was due to localised artefacts in specific humidity at high altitude / low pressure levels (50 hPa or 150 hPa). Our work thus further highlights the ever-present importance of careful data science in the deployment of large-scale deep learning models, and advocates for the use of multiple complementary metrics \citep{ravuri2021nowcasting} to assess the quality of models with applications to weather and climate modeling.

==> figure_hyper_prior_hurricane_matthew.tex <==
\begin{figure}
    %\centering
    \begin{flushright}
    \includegraphics[width=\textwidth, trim = 6cm 2.5cm 5cm 4.5cm, clip]{figures/experiments/hurricane_matthew/2016_10_5-0_HyperPrior_temperature_850hPa.pdf}
    \includegraphics[width=\textwidth, trim = 6cm 2.5cm 5cm 4.5cm, clip]{figures/experiments/hurricane_matthew/2016_10_5-0_HyperPrior_specific_humidity_1000hPa.pdf}
    \includegraphics[width=\textwidth, trim = 6cm 2.5cm 5cm 4.5cm, clip]{figures/experiments/hurricane_matthew/2016_10_5-0_HyperPrior_u_component_of_wind_1000hPa.pdf}
    \includegraphics[width=\textwidth, trim = 6cm 3.8cm 5cm 2.8cm, clip]{figures/experiments/hurricane_matthew/2016_10_5-0_HyperPrior_u_component_of_wind_zoom_1000hPa.pdf}
    % \includegraphics[width=\textwidth, trim = 6cm 2.5cm 5cm 4.5cm, clip]{figures/experiments/hurricane_matthew/2016_10_5-0_HyperPrior_geopotential_500hPa.pdf}
    \includegraphics[width=\textwidth, trim = 6cm 3.8cm 5cm 2.8cm, clip]{figures/experiments/hurricane_matthew/2016_10_5-0_HyperPrior_geopotential_zoom_500hPa.pdf}
    \includegraphics[width=0.65\textwidth, trim = 20cm 3.8cm 5cm 2.8cm, clip]{figures/baseline/2016_10_5-0_baseline_512_geopotential_zoom_500hPa.pdf}
    % \hspace*{-10em}
    \caption{Hyperprior reconstructions of a global frame on 2016/10/5 at 0 UTC, compressed $1000\times$. From top to bottom: temperature at 850 hPa, specific humidity at 1000 hPa, the zonal component of wind at 1000 hPa (and a zoom over the Caribbean), and geopotential at 500 hPa over the Caribbean. Last row shows reconstruction using \citet{huang2022compressing} compressed $1150\times$ as a baseline. Columns show the ground truth, the reconstruction and the residual along mean absolute error (MAE). Note the improvement in Hurricane Matthew's reconstruction over the baseline.}
    \label{fig:hurricane_matthew_hyperprior}
    \end{flushright}
\end{figure}

==> paper_planning.tex <==

\section{Paper planning}

\subsection{Story}
\subsubsection{Problem}

Much of climate science depends on historical atmospheric datasets like ERA5. However, their PB-scale size costs \$ $X$ to keep on a datacenter, which can be prohibitive to the majority of the scientific community. With scientific demand for ever higher resolution, this problem is set to worsen at a pace that far outstrips the palliative effects of Moore's Law. The usual workaround by researchers is to give up and sample sparsely from such datasets, potentially leaving many insights on the cutting-room table.

\subsubsection{Solution} 
We compress atmospheric datasets from datacenter-scale to desktop SSD scale, thus enabling researchers to use them in full.

\subsubsection{How this is new and different}
\begin{enumerate}
\item We learn the compressor, fitting our representation to the dataset unlike [...].
\item We validate our work on a large portion of ERA5's frames, and all channels, unlike [...].
\item Our validation measures not just MSE and PSNR, but also the frequency distribution, unlike [...].
\item Across the above measures, we are SOTA.
\end{enumerate}

\subsection{Results}
\subsubsection{Our claims}
%We make the following claims:
\begin{enumerate}
    \item \textbf{Global spatial error:} Across the test set, our models have lower error in cartesian space than the competition.
    \begin{enumerate}
        \item MSE
        \item Max
        \item \% "bad pixels" (top N-percentile error)
        \item All of the above, but in a spatiotemporal window around extreme events (e.g. in the Caribbean, during famous hurricanes there).
    \end{enumerate}
    \item \textbf{Global frequency error:} Across the test set, our models have lower error in frequency space than the competition.
    \item \textbf{Rare events:} Our model gets lower \textbf{\emph{local}} spatial error on rare events (example: local heatwaves, hurricanes) than competing models.
\end{enumerate}

\subsubsection{Evidence for our claims}
\begin{enumerate}
    \item Evidence for \textbf{global spatial error} claim:
    \begin{enumerate}
        \item \textbf{MSE vs compression ratio plot}
        \item[] Show one curve for each of our models (HP, FP, VQVAE, VQGAN), and single points for competing models.
        \begin{itemize}
            \item $X$ axis: the compression ratio. 
            \item $Y$ axis: MSE over all pixels and all frames in the test set. 
            \item The competing models may need asterisks describing differences in their datasets to ours, for example "* geopotential only". This apples-and-oranges difference may be fine so long as we outperform them on the harder task of measuring on the full test set across all channels (as opposed to them only compressing geopotential on one frame).
        \end{itemize}
        \item \textbf{MSE quantiles plot}
        \item[] MSE quantile plots, transposed to act as plots of the MSE distribution (CDF).
        \begin{itemize}
            \item One plot with 5 curves, one for each channel in the vertical levels dataset. \newline $X$ axis: normalized error at quantile boundaries, with denser sampling near the extremes, e.g. [0\%, .001\%, .01\%, .1\%, 1\%, 10\%, 20\%, [...], 80\%, 90\%, 99\%, 99.9\%, 99.99\%, 99.999\%, 100\%] (axis should be just the absolute error value). 
            \item $Y$ axis: \% of pixels whose error is less than the quantile boundary at $x$. 
            \item Supporting table: show the un-normalized sensor values corresponding to the quantile boundaries. 5 columns, one for each channel. N rows, one for each quantile boundary. The first and last rows will show the min and max errors for that channel across the whole dataset; emphasize this point.
        \end{itemize}
    \item \textbf{PSNR plot (optional)}
    \item[] Reviewers from image compression may ask for this. Until they do, don't bother. (Easy enough to add it to the eval pipeline.)
    \end{enumerate}
    
    \item Evidence for \textbf{global frequency error} claim:
    \begin{enumerate}
        \item Spherical harmonic error plot. 
        \item[] The new hotness replacing RAPSD plots. Piotr recommends a simple 2D plot of wavelength vs power, like RAPSD. A 3D surface. Show one plot per model, including competitors' models.
        \begin{itemize}
            \item X axis: \# of zero-crossings in longitudinal direction.
            \item Y axis: \# of zero-crossings in latitudinal direction.
            \item Z axis: $R_{i,j} - D_{i, j}$, where $R_{i,j}$ is the reconstruction's frequency response, and $D_{i,j}$ is the original data's frequency response, to the $(i, j)$'th spherical harmonic. Color coded: 0 = black, positive: blue, negative: red
            \item If these plots turn out to be mostly radially symmetric in the x-y plane, consider taking the average over theta in polar coordinates, to convert them to RAPSD-style 2D curves that plot power vs frequency. Curves are much easier to read than 3D surfaces. This would allow us to plot all models' curves on one plot. Note that despite the visual similarity to RAPSD, this is still a big improvement over it, since it's measured over the whole earth, not a single healpix square with awkward hacks to work around the edges.
        \end{itemize} 
    \end{enumerate}
    
    \item Evidence for \textbf{rare events} claim:
    \begin{enumerate}
        \item MSE vs value plot.
        \item[] This measures the pixelwise reconstruction error, as a function of pixel value intensity. A model that reconstructs large values poorly does not preserve extreme events well.
        \begin{itemize}
            \item $X$ axis: log(absolute normalized value) (range: $[0, log(v_{max}/\sigma)]$).
            \item $Y$ axis: MSE over all pixels and all frames in test set with that value.
            \item Plot multiple curves on a single plot, one curve per model (including competitors). Curves should show variance envelopes. For models that compress extreme values poorly, the curve will go up and to the right. 
        \end{itemize}
        \item Screenshot of bad and good hurricane reconstruction.
        \item[] as an example here, show the figure 9 of~\cite{hoefler2023earth} in figure~\ref{fig:hurricane_matthew_hoefler2023earth} with disappearing hurricane for NN and preserved hurricane in SZ3.
        
        \begin{figure}[ht]
            \centering
            % Replace 'example-image' with the path to your actual image file
            \includegraphics[width=0.7\textwidth]{assets/ref_nn_sz3_hurricane_matthew_hoefler2023}
            \caption{\cite{hoefler2023earth} achieve high compression ratios, which comes at the expense of recovering extreme events }
            \label{fig:hurricane_matthew_hoefler2023earth}
        \end{figure}
    \end{enumerate}
\end{enumerate}


\subsubsection{Ablations}
%We make the following claims:
\begin{enumerate}
    \item \textbf{Padding:} Our padding + interpolation results in quantitative and qualitative improvements (supressing seams).
    \item \textbf{Hyperparameter choices:} Our models are well tuned.
\end{enumerate}


\subsubsection{Ablations description}
\begin{enumerate}
    \item Ablations for \textbf{padding} choice:
    \begin{enumerate}
        \item TODO
        \begin{itemize}
            \item TODO
        \end{itemize}
    \end{enumerate}
    
    \item Ablations for \textbf{hyperparameter} choice:
    \begin{enumerate}
        \item TODO
        \begin{itemize}
            \item TODO
        \end{itemize} 
    \end{enumerate}
\end{enumerate}

\subsubsection{Contributions}
\begin{enumerate}
    \item Open-source code?
    \item Open-source trained model + compressed ERA5?
    \item Open-source colab that uses the above trained model?
\end{enumerate}


\section{Unimportant TODOs, in decreasing order}
\begin{itemize}
    \item VITVQ
    \item FSQ (Finite Scalar Quantization)
\end{itemize}
